MPTCP meets FEC: Supporting Latency-Sensitive Applications over Heterogeneous Networks

Over the past years, TCP has gone through numerous updates to provide performance enhancement under diverse network conditions. However, with respect to losses, little can be achieved with legacy TCP detection and recovery mechanisms. Both fast retransmission and retransmission timeout take at least one extra round trip time to perform, and this might significantly impact performance of latency-sensitive applications, especially in lossy or high delay networks. While forward error correction (FEC) is not a new initiative in this direction, the majority of the approaches consider FEC inside the application. In this paper, we design and implement a framework, where FEC is integrated within TCP. Our main goal with this design choice is to enable latency sensitive applications over TCP in high delay and lossy networks, but remaining application agnostic. We further incorporate this design into multipath TCP (MPTCP), where we focus particularly on heterogeneous settings, considering the fact that TCP recovery mechanisms further escalate head-of-line blocking in multipath. We evaluate the performance of the proposed framework and show that such a framework can bring significant benefits compared to legacy TCP and MPTCP for latency-sensitive real application traffic, such as video streaming and web services.

==> applications.tex <==
\section{Latency-Sensitive Application Traffic}
The following Sections~\ref{subsection:http} and \ref{subsection:video} picture some of the main characteristics of the applications and application protocols used in the evaluation of this work. We emphasise the fact here, that these are very, if not the most, relevant ones in today's users Internet and mobile Internet reality.

\subsection{HTTP}\label{subsection:http}
%https://http2.github.io/faq/#why-revise-http
HTTP/1.1 has served the Internet now for more than 15 years, although loading web pages efficiently nowadays is more resource intensive and difficult. HTTP/1.1 practically allows only one outstanding request per TCP connection, and this led applications do data splitting, inlining, domain sharding and concatenation, to overcome problems in the protocol itself. To discuss it, HTTP/2 was developed by the IETF's HTTP Working Group, which also maintains HTTP/1.1.
\begin{enumerate}
    \item HTTP/1.1: Browsers have used multiple TCP connections to issue parallel requests. However, there are limits to this: First, if too many connections are used, TCP congestion control is effectively negated, leading to congestion that hurt performance. Second, it's fundamentally unfair, because browsers are taking more than their share of network resources, where certain browsers can open between four and eight connections per origin. At the same time, the large number of requests means a lot of duplicated data on the wire. Looking to these factors, HTTP/1.1 requests have an unnecessary related overhead and these can also end up hurting performance.
    \item HTTP/2: Instead of a textual protocol, HTTP/2 is fully multiplexed. It can also make multiple requests within a single TCP connection, therefore, using a single connection for parallelism. It also has header compression, reducing overhead allowing servers to push responses proactively into client caches.
\end{enumerate}

%HTTP/2: RFC 7540
\subsection{Video}\label{subsection:video}
%http://www.mediaentertainmentinfo.com/2015/04/6-concept-series-what-is-the-difference-between-progressive-download-rtmp-streaming-and-adaptive-streaming.html/
%https://en.wikipedia.org/wiki/Adaptive_bitrate_streaming#Adobe_Dynamic_Streaming_for_Flash
%http://www.streamingmedia.com/Articles/Editorial/Featured-Articles/RTMP-in-the-Age-of-HTTP-Video-Streaming-Dont-Count-it-Out-100909.aspx
Online video can be in form of live streaming or Video on Demand (VOD). In recent years, online video has taken a major leap with service providers having the challenging task to ensure seamless experience regardless of network conditions. Currently, three key technologies fill all segments of online video delivery: Progressive download, i.e., HTTP streaming over TCP, Real Time Messaging Protocol (RTMP) or Real Time Streaming Protocol (RTSP), i.e., chunk-based streaming and, finally, adaptive streaming majorly represented by Dynamic Adaptive Streaming over HTTP (DASH). These three models are technically different, but they are equally popular based on the nature of their end use, e.g., mobile Internet, Internet streaming, etc. 
%RTSP: RFC2326
%RTMP is RTMFP@IETF RFC7425

%http://www.onlinevideo.net/2011/05/streaming-vs-progressive-download-vs-adaptive-streaming
%http://www.globaldots.com/streaming-adobe-rtmp-explained/
\begin{enumerate}
    \item Progressive download: In opposite to classic download, server-based delivery over HTTP delivers (or buffers) a sufficient amount of the file on the end user's machine to immediately start the playback. Download of content happens sequentially and, hence, skipping ahead is not allowed. Progressive download gave feeling of streaming and reduced waiting times. However, it has some shortcomings: Security concerns, absence of monitoring and quality adjustment, restriction of linear playback and amount of wasted bandwidth for non-viewed content.
    \item RTMP/RTSP: This is content delivery mechanism used by specialised streaming servers, where nearly all live streaming events for in-browser desktop playback, require a video player that supports Flash-based rendering and RTMP playback. It offers content security through chunks without local caching. It also supports streaming of live content and, because these are stateful protocols, the server can detect environment changes and make transfer speed decisions to improve user experience.
    \item Adaptive streaming: This is the most popular form of video streaming with benefits of quality switching and ease of delivery over HTTP. It aggregates segments of multi-bit encoded videos in a manifest file. Client downloads the file and periodically requests for higher video quality. The flexibility to switch video segments based on CPU availability and network conditions, ensures un-interrupted playback. There are three established adaptive streaming technologies: Adobe's HTTP Dynamic Streaming (HDS), Apple's HTTP Live Streaming (HLS), Microsoft's Smooth Streaming and the specification from MPEG standards body, MPEG-DASH.
\end{enumerate}

In addition to HTTP and adaptive and non-adaptive video, we also include bulk traffic in our evaluation, the most common application evaluated with MPTCP.
